InstructExcel: A Benchmark for Natural Language Instruction in Excel

With the evolution of Large Language Models (LLMs) we can solve increasingly more complex NLP tasks across various domains, including spreadsheets. This work investigates whether LLMs can generate code (Excel OfficeScripts, a TypeScript API for executing many tasks in Excel) that solves Excel specific tasks provided via natural language user instructions. To do so we introduce a new large-scale benchmark, InstructExcel, created by leveraging the 'Automate' feature in Excel to automatically generate OfficeScripts from users' actions. Our benchmark includes over 10k samples covering 170+ Excel operations across 2,000 publicly available Excel spreadsheets. Experiments across various zero-shot and few-shot settings show that InstructExcel is a hard benchmark for state of the art models like GPT-4. We observe that (1) using GPT-4 over GPT-3.5, (2) providing more in-context examples, and (3) dynamic prompting can help improve performance on this benchmark.

==> pseudocode_data_aug.tex <==
\begin{algorithm}[t]
    \caption{Data Augmentation}
    \begin{algorithmic}
    %     \Require {Training data $\mathcal{T} = \{(M_i, I_i, O_i)\}_{1 \leq i \leq n}$ with metadata $\mathcal{M}$, NL inputs $\mathcal{I}$, and code outputs $\mathcal{O}$; list of methods present in each output $F = \{f_1, f_2, \dots f_n\}$; number of examples per prompt $\phi$; sampling ratio $\gamma$; target ratio $\tau$.}
    %     \State $\mathcal{T}_{aug} \gets \emptyset$
        
    %     \While{minMethodCount($\mathcal{O} \cup \mathcal{O}_{aug}$) < $\tau$ maxMethodCount($\mathcal{O} \cup \mathcal{O}_{aug}$)}
    %         \State Set $(M_i, I_i, O_i)$ to be an example with the least frequent method

    %         \State $\mathcal{T}_{prompt} \gets \emptyset$
        
    %         \For{$(M_j, I_j, O_j) \in \mathcal{T}$ in descending order by $\frac{|f_j \cap f_i|}{|f_j \cup f_i|}$, until $|\mathcal{T}_{prompt}| < \phi$}
    %             \State Put $(M_j, I_j, O_j)$ in $\mathcal{T}_{prompt}$ with probability $\gamma$
    %         \EndFor

    %         \State Shuffle $\mathcal{T}_{prompt}$
    %         \State Append $(M_i, I_i, O_i)$ to end of $\mathcal{T}_{prompt}$ (optional step)
            
    %         \State Generate input $I'_i$ by prompting GPT-3 with instruction, examples in $\mathcal{T}_{prompt}$, then $O_i$
    %         \State Append $(M_i, I'_i, O_i)$ to $\mathcal{T}_{aug}$
    %     \EndWhile
    % \State \Return $T_{aug}$
        \Require {Training data $\mathcal{T} = \{(M_i, I_i, O_i)\}_{1 \leq i \leq n}$ (metadata $M_i$, NL input $I_i$, code output $O_i$).}
        
        \State Select $(M_i, I_i, O_i)$ where $O_i$ contains the least frequently-used API method

        \State Select prompting examples $\mathcal{T}_{prompt}$ by sampling examples $(M_j, I_j, O_j)$ (sample probabilities are proportional to the Jaccard similarity in methods present in $O_i$ and $O_j$)
    
        % \For{$(M_j, I_j, O_j) \in \mathcal{T}$ in descending order by $\frac{|f_j \cap f_i|}{|f_j \cup f_i|}$, until $|\mathcal{T}_{prompt}| < \phi$}
        %     \State Put $(M_j, I_j, O_j)$ in $\mathcal{T}_{prompt}$ with probability $\gamma$
        % \EndFor

        \State (Optional) Append $(M_i, I_i, O_i)$ to $\mathcal{T}_{prompt}$
        
        \State Generate input $I'_i$ by prompting GPT-3 with instruction, examples in $\mathcal{T}_{prompt}$, then $O_i$
    \State \Return $(M_i, I'_i, O_i)$
    \end{algorithmic}
    \label{alg:data_aug}
  \end{algorithm}
